Dealing with observability in interaction-based Offline Runtime Verification of Distributed Systems

Interactions are formal models describing asynchronous communications within a Distributed System (DS). They can be drawn in the fashion of sequence diagrams and executed thanks to an operational semantics akin to that of process algebras. Executions of DS can be characterized by tuples of local traces (one per subsystem) called multi-traces. For a given execution, those local traces can be collected via monitoring and the resulting multi-trace can be analysed using offline Runtime Verification (RV). To that end, interactions may serve as formal references. In practice, however, not all subsystems may be observed and, without synchronising the end of monitoring on different subsystems, some events may not be observed, e.g. the reception of a message may be observed but not the corresponding emission. So as to be able to consider all such cases of partial observation, we propose an offline RV algorithm which uses removal operations to restrict the reference interaction on-the-fly, disregarding the parts concerning no longer observed subsystems. We prove the correctness of the algorithm and assess the performance of an implementation.

==> appendices/A6_table.tex <==
\begin{tabular}{|l|c|c|c|c|}
\hline
%\makecell{\footnotesize model}
&
\makecell{
Book Order \cite{coping_with_bad_agent_interaction_protocols_when_monitoring_partially_observable_multiagent_systems_AnconaFFM18}
}
&
\makecell{
Sensor Data \cite{a_dynamic_and_context_aware_semantic_mediation_service_for_discovering_and_fusion_of_heterogeneous_sensor_data}
}
&
\makecell{
ABP \cite{high_level_message_sequence_charts}
}
&
\makecell{
Network \cite{comprehensive_multiparty_session_types}
}
\\
% \hline
% % how the exploration
% \makecell{\footnotesize Exploration criteria}
% &
% \makecell{\scriptsize loop $\leq 2$\\\scriptsize exhaustive}
% &
% \makecell{\scriptsize loop $\leq 3$\\\scriptsize exhaustive}
% &
% \makecell{\scriptsize loop $\leq 15$\\\scriptsize partial \& random\\\scriptsize node $\leq 40~000$}
% &
% \makecell{\scriptsize loop $\leq 6$\\\scriptsize exhaustive}
% \\
\hline
% number of accepted multi-traces
%\makecell{\rotatebox[origin=c]{90}{$|T_C(i)|$}}
%\makecell{\footnotesize $|T(i)|$}
\makecell{\footnotesize \#accepted multi-traces}
&
\makecell{$504$}
&
\makecell{$2~101$}
&
\makecell{$1~219$}
&
\makecell{$4~096$}
\\
\hline
% how the slices are made
%\makecell{\footnotesize \# prefixes \\ per trace}
%&
%\makecell{\scriptsize $20$ random prefixes\\\scriptsize per trace}
%&
%\makecell{\scriptsize $30$ random prefixes\\\scriptsize per trace}
%&
%\makecell{\scriptsize $20$ random prefixes\\\scriptsize per trace}
%&
%\makecell{\scriptsize $20$ random prefixes\\\scriptsize per trace}
%\\
%\hline
% number of slices
%\makecell{\rotatebox[origin=c]{90}{$|\sliceOf{T_C(i)}|$}}
%\makecell{\footnotesize $|P(i)|$}
\makecell{\footnotesize \# multi-prefixes }
&
\makecell{$10~452$}
&
\makecell{$65~121$}
&
\makecell{$25~599$}
&
\makecell{$85~948$}
\\
\hline
% size of slices
\makecell{\footnotesize size of multi-prefixes}
&
\makecell{$[0-20]$}
&
\makecell{$[0-54]$}
&
\makecell{$[72-204]$}
&
\makecell{$[0-48]$}
\\
\hline
\end{tabular}

==> figures/sensor/data.tex <==
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
{}
& {\scriptsize$0$-$50$} & {\scriptsize$51$-$100$} & {\scriptsize$101$-$150$} & {\scriptsize$151$-$350$} & {\scriptsize$351$-$700$} & {\scriptsize$701$\texttt{+}}\\
\hline
\rotatebox[origin=c]{90}{\textbf{\scriptsize \textcolor{green}{$\blacksquare$}}{\tiny rmv}}
%\textbf{\scriptsize \textcolor{green}{$\blacksquare$}} 
& \makecell{
\scriptsize$0.01558$\\
\scriptsize$0.01562$\\
\scriptsize$3.49917$\\
\scriptsize$47$NA} 
& \makecell{
\scriptsize$0.01464$\\
\scriptsize$0.01562$\\
\scriptsize$7.43576$\\
\scriptsize$95$NA} 
& \makecell{
\scriptsize$0.01561$\\
\scriptsize$0.01562$\\
\scriptsize$9.90544$\\
\scriptsize$95$NA} 
& \makecell{
\scriptsize$0.0156$\\
\scriptsize$0.0157$\\
\scriptsize$5.1238$\\
\scriptsize$354$NA} 
& \makecell{
\scriptsize$0.0156$\\
\scriptsize$0.0313$\\
\scriptsize$8.4347$\\
\scriptsize$422$NA} 
& \makecell{
\scriptsize$0.04687$\\
\scriptsize$0.06249$\\
\scriptsize$0.10195$\\
\scriptsize$92$NA}  \\
\hline
\rotatebox[origin=c]{90}{\textbf{\scriptsize \textcolor{blue}{$\blacksquare$}}{\tiny rmv\&loc}}
%\textbf{\scriptsize \textcolor{blue}{$\blacksquare$}} 
& \makecell{
\scriptsize$0.01558$\\
\scriptsize$0.01562$\\
\scriptsize$0.04687$\\
\scriptsize$0$NA} 
& \makecell{
\scriptsize$0.01410$\\
\scriptsize$0.02646$\\
\scriptsize$0.17254$\\
\scriptsize$0$NA} 
& \makecell{
\scriptsize$0.01559$\\
\scriptsize$0.04687$\\
\scriptsize$0.29677$\\
\scriptsize$0$NA} 
& \makecell{
\scriptsize$0.01559$\\
\scriptsize$0.04388$\\
\scriptsize$1.36437$\\
\scriptsize$0$NA} 
& \makecell{
\scriptsize$0.01559$\\
\scriptsize$0.40615$\\
\scriptsize$2.59121$\\
\scriptsize$0$NA} 
& \makecell{
\scriptsize$0.01559$\\
\scriptsize$0.04682$\\
\scriptsize$4.25371$\\
\scriptsize$0$NA}  \\
\hline
\rotatebox[origin=c]{90}{\textbf{\scriptsize \textcolor{red}{$\blacksquare$}}{\tiny sim}}
%\textbf{\scriptsize \textcolor{red}{$\blacksquare$}} 
& \makecell{
\scriptsize$0.01559$\\
\scriptsize$0.01562$\\
\scriptsize$9.16975$\\
\scriptsize$91$NA} 
& \makecell{
\scriptsize$0.01559$\\
\scriptsize$0.01563$\\
\scriptsize$8.75035$\\
\scriptsize$119$NA} 
& \makecell{
\scriptsize$0.01561$\\
\scriptsize$0.03124$\\
\scriptsize$8.06315$\\
\scriptsize$105$NA} 
& \makecell{
\scriptsize$0.0156$\\
\scriptsize$0.0312$\\
\scriptsize$9.7008$\\
\scriptsize$366$NA} 
& \makecell{
\scriptsize$0.0156$\\
\scriptsize$0.1934$\\
\scriptsize$9.2634$\\
\scriptsize$421$NA} 
& \makecell{
\scriptsize$0.06247$\\
\scriptsize$0.08548$\\
\scriptsize$5.73870$\\
\scriptsize$94$NA}  \\
\hline
\rotatebox[origin=c]{90}{\textbf{\scriptsize \textcolor{yellow}{$\blacksquare$}}{\tiny sim\&loc}}
%\textbf{\scriptsize \textcolor{yellow}{$\blacksquare$}} 
& \makecell{
\scriptsize$0.01559$\\
\scriptsize$0.01562$\\
\scriptsize$0.06249$\\
\scriptsize$0$NA} 
& \makecell{
\scriptsize$0.01559$\\
\scriptsize$0.02592$\\
\scriptsize$0.25792$\\
\scriptsize$0$NA} 
& \makecell{
\scriptsize$0.01561$\\
\scriptsize$0.04687$\\
\scriptsize$0.39050$\\
\scriptsize$0$NA} 
& \makecell{
\scriptsize$0.01559$\\
\scriptsize$0.03590$\\
\scriptsize$1.56962$\\
\scriptsize$0$NA} 
& \makecell{
\scriptsize$0.01559$\\
\scriptsize$0.40615$\\
\scriptsize$2.70205$\\
\scriptsize$0$NA} 
& \makecell{
\scriptsize$0.01559$\\
\scriptsize$0.04798$\\
\scriptsize$3.99155$\\
\scriptsize$0$NA}  \\
\hline
\end{tabular}

==> figures/sensor/hid_noloc.tex <==
\begin{Verbatim}[fontsize=\scriptsize]
> "number of times the timeout is exceeded using hiding without local analyses : 1105"
> "time summary at length category 0-50 using hiding without local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.    NA's 
0.01558 0.01562 0.01562 0.04460 0.01562 3.49917      47 
> "time summary at length category 51-100 using hiding without local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.    NA's 
0.01464 0.01562 0.01562 0.04265 0.01562 7.43576      95 
> "time summary at length category 101-150 using hiding without local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.    NA's 
0.01561 0.01562 0.01562 0.06107 0.01563 9.90544      95 
> "time summary at length category 151-350 using hiding without local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.    NA's 
 0.0156  0.0156  0.0157  0.0484  0.0312  5.1238     354 
> "time summary at length category 351-700 using hiding without local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.    NA's 
 0.0156  0.0312  0.0313  0.0708  0.0469  8.4347     422 
> "time summary at length category 701+ using hiding without local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.    NA's 
0.04687 0.06248 0.06249 0.06970 0.07627 0.10195      92 
\end{Verbatim}

==> figures/sensor/hid_wtloc.tex <==
\begin{Verbatim}[fontsize=\scriptsize]
> "number of times the timeout is exceeded using hiding with local analyses : 0"
> "time summary at length category 0-50 using hiding with local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max. 
0.01558 0.01562 0.01562 0.01980 0.01565 0.04687 
> "time summary at length category 51-100 using hiding with local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max. 
0.01410 0.01562 0.02646 0.04283 0.06249 0.17254 
> "time summary at length category 101-150 using hiding with local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max. 
0.01559 0.01562 0.04687 0.08048 0.14059 0.29677 
> "time summary at length category 151-350 using hiding with local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max. 
0.01559 0.01562 0.04388 0.21080 0.35929 1.36437 
> "time summary at length category 351-700 using hiding with local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max. 
0.01559 0.02298 0.40615 0.55760 0.99977 2.59121 
> "time summary at length category 701+ using hiding with local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max. 
0.01559 0.03124 0.04682 1.14983 2.13609 4.25371 
\end{Verbatim}

==> figures/sensor/sim_noloc.tex <==
\begin{Verbatim}[fontsize=\scriptsize]
> "number of times the timeout is exceeded using simulation without local analyses : 1196"
> "time summary at length category 0-50 using simulation without local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.    NA's 
0.01559 0.01562 0.01562 0.08921 0.01563 9.16975      91 
> "time summary at length category 51-100 using simulation without local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.    NA's 
0.01559 0.01562 0.01563 0.09329 0.03124 8.75035     119 
> "time summary at length category 101-150 using simulation without local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.    NA's 
0.01561 0.01562 0.03124 0.10834 0.03124 8.06315     105 
> "time summary at length category 151-350 using simulation without local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.    NA's 
 0.0156  0.0312  0.0312  0.2376  0.0833  9.7008     366 
> "time summary at length category 351-700 using simulation without local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.    NA's 
 0.0156  0.0469  0.1934  0.9106  1.2770  9.2634     421 
> "time summary at length category 701+ using simulation without local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.    NA's 
0.06247 0.06249 0.08548 0.51048 0.51148 5.73870      94 
\end{Verbatim}


==> figures/sensor/sim_wtloc.tex <==
\begin{Verbatim}[fontsize=\scriptsize]
> "number of times the timeout is exceeded using simulation with local analyses : 0"
> "time summary at length category 0-50 using simulation with local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max. 
0.01559 0.01562 0.01562 0.02152 0.03123 0.06249 
> "time summary at length category 51-100 using simulation with local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max. 
0.01559 0.01562 0.02592 0.05053 0.07811 0.25792 
> "time summary at length category 101-150 using simulation with local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max. 
0.01561 0.01562 0.04687 0.09326 0.15621 0.39050 
> "time summary at length category 151-350 using simulation with local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max. 
0.01559 0.01562 0.03590 0.22555 0.38231 1.56962 
> "time summary at length category 351-700 using simulation with local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max. 
0.01559 0.01565 0.40615 0.56170 1.01538 2.70205 
> "time summary at length category 701+ using simulation with local analyses :"
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max. 
0.01559 0.03124 0.04798 1.16043 2.20405 3.99155 
\end{Verbatim}

==> figures/sensor/timeout.tex <==
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
{\tiny meth\textbackslash len}
& {\scriptsize$0$-$50$} & {\scriptsize$51$-$100$} & {\scriptsize$101$-$150$} & {\scriptsize$151$-$350$} & {\scriptsize$351$-$700$} & {\scriptsize$701$\texttt{+}}\\
\hline
\textbf{\scriptsize \textcolor{green}{$\blacksquare$}}{\tiny rmv} & {\scriptsize$47$} & {\scriptsize$95$} & {\scriptsize$95$} & {\scriptsize$354$} & {\scriptsize$422$} & {\scriptsize$92$} \\
\hline
\textbf{\scriptsize \textcolor{blue}{$\blacksquare$}}{\tiny rmv\&loc} & {\scriptsize$0$} & {\scriptsize$0$} & {\scriptsize$0$} & {\scriptsize$0$} & {\scriptsize$0$} & {\scriptsize$0$} \\
\hline
\textbf{\scriptsize \textcolor{red}{$\blacksquare$}}{\tiny sim} & {\scriptsize$91$} & {\scriptsize$119$} & {\scriptsize$105$} & {\scriptsize$366$} & {\scriptsize$421$} & {\scriptsize$94$} \\
\hline
\textbf{\scriptsize \textcolor{yellow}{$\blacksquare$}}{\tiny sim\&loc} & {\scriptsize$0$} & {\scriptsize$0$} & {\scriptsize$0$} & {\scriptsize$0$} & {\scriptsize$0$} & {\scriptsize$0$} \\
\hline
\end{tabular}

==> figures/subfig/tikz_glotrace.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt}]
    \node (lab) {\texttt{trace}};
    \node[below=.1cm of lab] (lab2) {\scriptsize(\texttt{global})};
    \node[below=.1cm of lab2] (img) {\includegraphics[height=.9cm]{images/icons/icon_text_file.png}};
\end{tikzpicture}

==> figures/subfig/tikz_l1.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt}]
    \node (lab) {\texttt{\hlf{pub}}};
    \node[below=.1cm of lab] (img) {\includegraphics[height=1.4cm]{images/icons/icon_device.png}};
\end{tikzpicture}

==> figures/subfig/tikz_l2.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt}]
    \node (lab) {\texttt{\hlf{bro}}};
    \node[below=.1cm of lab] (img) {\includegraphics[width=1.6cm]{images/icons/icon_server.png}};
\end{tikzpicture}

==> figures/subfig/tikz_l3.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt}]
    \node (lab) {\texttt{\hlf{sub}}};
    \node[below=.1cm of lab] (img) {\includegraphics[height=1.3cm]{images/icons/icon_smartphone.png}};
\end{tikzpicture}

==> figures/subfig/tikz_loctrace.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt}]
    \node (lab) {\texttt{trace}};
    \node[below=.1cm of lab] (lab2) {\scriptsize(\texttt{local})};
    \node[below=.1cm of lab2] (img) {\includegraphics[height=.9cm]{images/icons/icon_text_file.png}};
\end{tikzpicture}

==> figures/subfig/tikz_loctrace_cmplt.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt}]
    \node (lab) {\scriptsize\texttt{local trace}};
    \node[below=.1cm of lab] (lab2) {\scriptsize(\texttt{complete})};
    \node[below=.1cm of lab2] (img) {\includegraphics[height=.9cm]{images/icons/icon_text_file.png}};
\end{tikzpicture}

==> figures/subfig/tikz_loctrace_partial.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt}]
    \node (lab) {\scriptsize\texttt{local trace}};
    \node[below=.1cm of lab] (lab2) {\scriptsize(\texttt{partial})};
    \node[below=.1cm of lab2] (img) {\includegraphics[height=.9cm]{images/icons/icon_text_file_partial.png}};
\end{tikzpicture}

==> figures/subfig/tikz_pub_bro_sub.tex <==
\begin{tikzpicture}
\tikzstyle{subsys}=[draw,hibou_col_lf,rectangle,line width=2pt,minimum height=2cm,minimum width=2cm,inner sep=0,outer sep=0]
%
\node[subsys] (A) at (-1.5,0) {
    \input{figures/subfig/tikz_l1}
};
%
\node[subsys] (B) at (1.5,1.5) {
    \input{figures/subfig/tikz_l2}
};
%
\node[subsys] (C) at (1.25,-1) {
    \input{figures/subfig/tikz_l3}
};
%
\draw[<->,line width=2.5pt,hibou_col_ms] (A) -- (B);
\draw[<->,line width=2.5pt,hibou_col_ms] (A) -- (C);
\draw[<->,line width=2.5pt,hibou_col_ms] (C) -- (B);
\end{tikzpicture}

==> figures/subfig/tikz_reord.tex <==
\begin{tikzpicture}[every node/.style={minimum height=0pt,minimum width=0pt}]
    \node (lab) {\texttt{reordering}};
    \node[below=.1cm of lab] (img) {\includegraphics[height=1.3cm]{images/icons/icon_ordering.png}};
\end{tikzpicture}
